Debiasing Neighbor Aggregation for Graph Neural Network in Recommender Systems

Graph neural networks (GNNs) have achieved remarkable success in recommender systems by representing users and items based on their historical interactions. However, little attention was paid to GNN's vulnerability to exposure bias: users are exposed to a limited number of items so that a system only learns a biased view of user preference to result in suboptimal recommendation quality. Although inverse propensity weighting is known to recognize and alleviate exposure bias, it usually works on the final objective with the model outputs, whereas GNN can also be biased during neighbor aggregation. In this paper, we propose a simple but effective approach, neighbor aggregation via inverse propensity (Navip) for GNNs. Specifically, given a user-item bipartite graph, we first derive propensity score of each user-item interaction in the graph. Then, inverse of the propensity score with Laplacian normalization is applied to debias neighbor aggregation from exposure bias. We validate the effectiveness of our approach through our extensive experiments on two public and Amazon Alexa datasets where the performance enhances up to 14.2%.

==> 2-related_work2.tex <==
\section{Preliminary and Related Work}

\emph{Recommender systems} receive users' previous interactions with items and provide a list of items that each user would like.
To perform such personalized recommendation task, recommenders are trained to reconstruct the observed interactions among users and items so as to find similar user-item pairs, which is known as collaborative filtering~\cite{he2017neural}.
Formally, given a recommender model $\phi(\cdot)$ and its prediction for user $u$'s relevance on item $i$ as $\phi(u,i)$, the ideal training objective for the recommender $\phi$ is to minimize loss on implicit feedback $Y_{u,i}$ collected via unbiased policy $\pi$,
\begin{equation}
    R(\pi) = \mathbb{E}_{p(u,i|\pi)}[\mathcal{L}\big(\phi(u,i), Y_{u,i}\big)],
\label{eq:default_loss}
\end{equation}
% \begin{equation}
%     R(\pi) = \mathbb{E}_{(u,i)\sim\pi}[\mathcal{L}\big(\phi(u,i), Y_{u,i}\big)],
% \label{eq:default_loss}
% \end{equation}

where $\mathcal{L}$ is an objective function such as mean squared error or Bayesian personalized ranking\,\cite{rendle2012bpr}, and the implicit feedback $Y_{u,i}$ is $1$ if the interaction between user $u$ and item $i$ is observed or $0$ if not.
A prevalent approach for collaborative filtering follows two steps: \emph{(i)} transform each user and item into a latent representation, $h_u$ and $h_i$, then \emph{(ii)} exploit the representation to estimate the relevance $\phi(u,i)$ based on dot product\,\cite{rendle2012bpr} or non-linear neural networks\,\cite{he2017neural}.

\begin{definition}\,{\sc (Policy)}
\label{def:policy}
Policy $\pi$ is a prior that describes user behaviors in a system.
\end{definition}
\begin{definition}\,{\sc (Propensity)}
\label{def:propensity}
Propensity $p(Y_{u,i}\!=\!1|\pi)$ is the observation probability of user-item interaction $Y_{u,i}$ under policy $\pi$.
\end{definition}



% \begin{comment}
% 1. scoping into BPR to dribble readers
% 2. ordering of new notions. especially data collection related issues, right before method section
% 3. paragraph-wise main sentence

% \emph{Recommender systems} receive users' previous interactions with items and provide a list of items that each user would like.
% To perform such personalized recommendation task, recommenders are trained to minimize ranking loss~\cite{rendle2012bpr} so as to prioritize observed interactions among users and items over unobserved ones. 
% Formally, given a recommender model $\phi(\cdot)$ and its prediction for user $u$'s relevance on item $i$ as $\phi(u,i)$, the ideal training objective for the recommender $\phi$ is to minimize loss on implicit feedback $Y_{u,i}$ collected via unbiased policy $\pi$,
% \begin{equation}
%     R(\pi) = \mathbb{E}_{(u,i,j)\sim\pi}[Y_{u,i}(1-Y_{u,j})
%     ~\text{ln}\sigma\big(\phi(u,i)-\phi(u,j)\big)],
% \label{eq:default_loss}
% \end{equation}
% where $\mathcal{L}$ is an objective function such as mean squared error or Bayesian personalized ranking\,\cite{rendle2012bpr}, and the implicit feedback $Y_{u,i}$ is $1$ if the interaction between user $u$ and item $i$ is observed or $0$ if not.
% A prevalent approach for collaborative filtering is 1) to transform each user and item into a latent representation, $h_u$ and $h_i$, then 2) exploit the representation to estimate the relevance $\phi(u,i)$ based on dot product\,\cite{rendle2012bpr} or non-linear neural networks\,\cite{he2017neural}.
% \end{comment}

% To generate a latent representation $h$ for a target user or item, early collaborative filtering studies consider the target itself only. % avoid objective sentence being placed in front of a sentence
% data collection policy while explaining GNN?
% rec -> unbiase rec -> GNN? + unbiasing GNN?
% technically correct words (less focus on sales, at the moment) detail
% rw <- scientific finding
\subsection{GNN for Recommender System}
\label{sec:related_work_gnn}
To generate a latent representation $h$ for a target user or item, early collaborative filtering studies consider the target itself only.
%Graph Neural Network is one of state-of-art approach for learning representation over graph.
%The key idea of GNN is to exploit information neighbors as well as the target nodes to generate latent representation of the target node.
However, a target's connected neighbors can provide more information about the target.
In this regard, GNN exploits information of a target's connected neighbors to generate $h$.

Specifically, given a bipartite graph of users and items as nodes and their interactions by a data collection policy $\tilde{\pi}$, GNN augments the embedding of a target node based on its connected neighbors. 
For a user $u$, GNN augments the embedding of $u$ at layer $l$ as $h^{l}_{u}$, 
\begin{align}
h^{(l)}_{u} &= {\rm TRANSFORM}\big(h^{(l-1)}_{u}, a^{(l)}_{\mathcal{N}_{\tilde{\pi}}(u)} \big)
\label{eq:transformation}\\
% a^{(l)}_{\mathcal{N}_{\tilde{\pi}}(u)} &= {\rm AGGREGATE}\big(w_{u,i}*h^{(l-1)}_{i}, i \in \mathcal{N}_{\tilde{\pi}}(u) \wedge (u,i) \sim \tilde{\pi} \big),
a^{(l)}_{\mathcal{N}_{\tilde{\pi}}(u)} &= {\rm AGGREGATE}\big(w_{u,i}*h^{(l-1)}_{i}, i \in \mathcal{N}_{\tilde{\pi}}(u) \big),
\label{eq:aggregation}
\end{align}
where $a^{(l)}_{\mathcal{N}_u}$ denotes the aggregated embedding of $u$'s neighbor items ${i \in \mathcal{N}_{\tilde{\pi}}(u)}$. 
Note that we can augment the embedding of item $i$ in the same way. Likewise, subsequent explanations will be in terms of user throughout this paper to avoid the redundancy of notation.

Each GNN method designs two functions: $(i)$ ${\rm TRANSFORM(\cdot)}$ fuses the embeddings of target $h^{(l-1)}_{u}$ and aggregated neighbors $a^{(l)}_{\mathcal{N}_u}$, and $(ii)$ ${\rm AGGREGATE(\cdot)}$ combines embeddings of neighbors with $w_{u,i}$ as the neighbor weight for the during aggregation.
Typically, usual GNN sets graph Laplacian norm as $w_{u,i}$ in Eq.\eqref{eq:aggregation} for numerical instability issue;
symmetric normalized Laplacian\,\cite{kipf2016semi,zhang2021causal,he2020lightgcn} uses the target node's edge degree, $a^{(l)}_{\mathcal{N}_{\tilde{\pi}}(u)} = \mathbb{E}_{(u,i) \sim \tilde{\pi}}[\frac{1}{|\mathcal{N}_{u}|}*h_{i}^{l-1}]$,
while random walk normalized Laplacian\,\cite{hamilton2017inductive, xu2018powerful} uses both edge degree of target and neighbor nodes, $a^{(l)}_{\mathcal{N}_{\tilde{\pi}}(u)} = \mathbb{E}_{(u,i) \sim\tilde{\pi}}[\frac{1}{\sqrt{|\mathcal{N}_{u}||\mathcal{N}_{i}|}}*h_{i}^{l-1}]$.
However, both graph Laplacian norms make neighbor aggregation \emph{biased} because the data collection policy $\tilde{\pi}$ is known to be different from unbiased policy $\pi$\,\cite{swaminathan2015self}. 
For instance, random walk Laplacian norm of user $u$'s neighbor aggregation is driven as
\begin{equation}
a^{(l)}_{\mathcal{N}_{\tilde{\pi}}(u)} \neq a^{(l)}_{\mathcal{N}_{\pi}(u)} = \mathbb{E}_{(u,i) \sim \pi}\big[\frac{1}{|\mathcal{N}_{u}|}*h_{i}^{l-1}\big].
\end{equation}
\begin{comment}
For instance, random walk Laplacian norm of user $u$'s neighbor aggregation is driven as
\begin{align}
a^{(l)}_{\mathcal{N}_{\tilde{\pi}}(u)} &= \mathbb{E}_{(u,i) \sim \tilde{\pi}}\big[\frac{1}{|\mathcal{N}_{u}|}*h_{i}^{l-1}\big] \label{eq:biased_neighbor_aggregation} \\
\neq a^{(l)}_{\mathcal{N}_{\pi}(u)} &= \mathbb{E}_{(u,i) \sim \pi}\big[\frac{1}{|\mathcal{N}_{u}|}*h_{i}^{l-1}\big].
\end{align}
\end{comment}
The neighbor bias $|a^{(l)}_{\mathcal{N}_{\tilde{\pi}}(u)} - a^{(l)}_{\mathcal{N}_{\pi}(u)}|$ is maintained throughout the entire optimization process once $w_{u,i}$ is fixed.
On the other hand, learnable neighbor aggregators such as attention\,\cite{velivckovic2017graph} or LSTM\,\cite{hamilton2017inductive} also become biased to $\tilde{\pi}$ during training because the aggregator minimizes empirical risk in the given biased policy $\tilde{\pi} \neq \pi$.

\begin{comment}

\begin{align}
a^{(l)}_{\mathcal{N}_{\tilde{\pi}}(u)} &= {\rm AGGREGATE}\big(w_{u,i}*h^{(l-1)}_{i}, i \in \mathcal{N}_{\tilde{\pi}}(u) \wedge (u,i) \sim \tilde{\pi} \big)\\
a^{(l)}_{\mathcal{N}_{\pi}(u)} &= {\rm AGGREGATE}\big(w_{u,i}*h^{(l-1)}_{i}, i \in \mathcal{N}_{\pi}(u) \wedge (u,i) \sim \pi \big),
\end{align}

\begin{equation}
w_{u,i}=
    \begin{cases}
    \frac{1}{|\mathcal{N}_{u}|} & \text{if}\quad w_{u,i}=L^{sym}_{u,i}\\ 
    \frac{1}{\sqrt{|\mathcal{N}_{u}||\mathcal{N}_{i}|}} & \text{if}\quad w_{u,i}=L^{rw}_{u,i},
    \end{cases}
\end{equation}
\end{comment}

\subsection{Inverse Propensity Scoring}
It is not feasible to perform learning on $R(\pi)$ as in Eq.\eqref{eq:default_loss} because data is collected via biased policy, $\tilde{\pi} \neq \pi$.
In this regard, inverse propensity scoring\,(IPS) fixes the data distribution mismatch between $\pi$ and $\tilde{\pi}$ via Monte Carlo approximation for loss function,
\begin{equation}
    \hat{R}(\pi)=\frac{1}{|\mathcal{D}|}\sum_{(u,i, Y_{u,i})\in \mathcal{D}}\frac{\mathcal{L}\big(\phi(u,i), Y_{u,i})\big)}{\tilde{\pi}(u,i)} \approx R(\pi),
\label{eq:IPS_loss}
\end{equation}
where $\mathcal{D} \sim \tilde{\pi}$, and $\tilde{\pi}(u,i)$ is the propensity score for user-item interaction $(u,i)$.
To this end, UBPR\,\cite{saito2019unbiased} exploits item popularity as propensity score $\tilde{\pi}(u,i)$ to make unbiased estimator $\hat{R}(\pi)$ for recommenders.
UEBPR\,\cite{damak2021debiased} improves UBPR with neighborhood based explainability that measures how much a target user's previously interacted items overlap with a target item's similar items. 
Moreover, AutoDebias approximates $\tilde{\pi}(u,i)$ via meta-learning based on uniformly collected data\,\cite{chen2021autodebias}.
However, because IPS methods work on the final objective, they do not explicitly handle how GNN aggregates neighbors.


\begin{comment}
\subsubsection{Causal Modeling}
Usually, recommender systems consider user and item as the only cause for user-item interactions.
However, user-item interactions are also affected by various confounding factors such as item popularity or exposure rate.
Consequently, recommenders cannot distinguish these confounders from pure user interest and provides unsatisfactory user experience.

In this regard, causal modeling methods first adds confounders of interest to causal graph as a variable for user-item interaction, then prunes or leverages their effect while modeling user interest.
For example, \cite{wang2021clicks} explicitly models exposure factor and remove its causal effect to mitigate clickbait issue.
DecRS\,\cite{wang2021deconfounded} regards confounder effect of imbalanced item distribution on user representation as the cause of bias amplification and removes them.
MACR\,\cite{wei2021model} first models direct causal relation from user and item toward preference score, and then prune their effect during inference to eliminate popularity bias.
DICE\,\cite{zheng2021disentangling} disentangles interest factor and popularity conformity factor. To this end, DICE learns two separate embedding vectors for each user and item, instead of one as in BPR\,\cite{rendle2012bpr}.
\end{comment}

==> 3-preliminary.tex <==

\section{Preliminary}
% \newcommand{}[1]{\boldsymbol{#1}}
\newcommand{\neighbor}[1]{\mathcal{N}_{#1}}
\newcommand{\user}{u}

% \section{Introduction}

% \section{Preliminary}
% \subsection{}
% \subsection{NGCF}
\subsubsection{Neighbor aggregation}
\begin{equation}
\begin{split}
    \boldsymbol{e}^{(k+1)}_{u}= \sigma\Big(\boldsymbol{W}_1\boldsymbol{e}^{(k)}_{u} + \sum_{i\in\neighbor{\user}}\frac{1}{\sqrt{\neighbor{\user}}\sqrt{\mathcal{N}_i}}\big(\boldsymbol{W}_1\boldsymbol{e}^{(k)}_{i}+\boldsymbol{W}_2(\boldsymbol{e}^{(k)}_{i}\odot \boldsymbol{e}^{(k)}_{u})\big)\Big)\\
    \boldsymbol{e}^{(k+1)}_{i}= \sigma\Big(\boldsymbol{W}_1\boldsymbol{e}^{(k)}_{i} + \sum_{u\in\mathcal{N}_i}\frac{1}{\sqrt{\mathcal{N}_i}\sqrt{\mathcal{N}_u}}\big(\boldsymbol{W}_1\boldsymbol{e}^{(k)}_{u}+\boldsymbol{W}_2(\boldsymbol{e}^{(k)}_{u}\odot \boldsymbol{e}^{(k)}_{i})\big)\Big)
\end{split}
\end{equation}
\subsubsection{Layer combination for model prediction (Concatenation)}
\begin{equation}
\begin{split}
    \boldsymbol{e}_{u}= \boldsymbol{e}^{(0)}_{u}||\cdots||\boldsymbol{e}^{(L)}_{u}\\
    \boldsymbol{e}_{i}= \boldsymbol{e}^{(0)}_{i}||\cdots||\boldsymbol{e}^{(L)}_{i}
\end{split}
\end{equation}

\subsection{LightGCN}
\subsubsection{Neighbor aggregation}
\begin{equation}
\begin{split}
    \boldsymbol{e}^{(k+1)}_{u}= \sum_{i\in\mathcal{N}_u}\frac{1}{\sqrt{\mathcal{N}_u}\sqrt{\mathcal{N}_i}}\boldsymbol{e}^{(k)}_{i}\\
    \boldsymbol{e}^{(k+1)}_{i}= \sum_{u\in\mathcal{N}_i}\frac{1}{\sqrt{\mathcal{N}_i}\sqrt{\mathcal{N}_u}}\boldsymbol{e}^{(k)}_{u}
\end{split}
\end{equation}
\subsubsection{Layer combination for model prediction (Sum)}
\begin{equation}
\begin{split}
    \boldsymbol{e}_{u}= \sum_{k=0}^{K}\alpha_k \boldsymbol{e}^{(k)}_{u}\\
    \boldsymbol{e}_{i}= \sum_{k=0}^{K}\alpha_k \boldsymbol{e}^{(k)}_{i}\\
\end{split}
\end{equation}

\newpage
\section{Method}
Idea: let's try weighted graph Laplacian on propensity score weighted graph and inverse propensity score weighted graph.

\newpage
\section{Analysis on GCN Normalization}
\subsection{Laplacian}
Suppose a graph $\mathcal{G}$ with $M+N$ nodes where $M$ is the number of users and $N$ is the number of items. Then, Laplacian matrix $L\in \mathcal{R}^{(M+N)\times(M+N)}$ is defined as $L = D - W$, where W is the weight matrix of $\mathcal{G}$ and $D$ is a diagonal degree matrix with each node degree as the sum of weights connected to it. Laplacian matrix $L$ is further (symmetrically) normalized $L^{sym} = D^{-\frac{1}{2}}LD^{-\frac{1}{2}}= I - D^{-\frac{1}{2}}WD^{-\frac{1}{2}}$ in transductive spectral convolution,
\begin{equation}
L^{sym}_{src, dst} =
\begin{cases}
1 & \text{if $src=dst$} \\
D^{-\frac{1}{2}}_{src}W_{src,dst}D^{-\frac{1}{2}}_{dst} & \text{if $src\neq dst$ and $(src,dst) \in \mathcal{D}$} \\
0 & \text{otherwise}.
\end{cases}
\label{eq:Laplacian_normalization}
\end{equation}


$L^{sym}_{src, dst}= D^{-1}_{src} W_{src,dst}$


In a typical GCN setting, adjacency matrix $A$ is used as weight matrix $W$, where all the weights for edges are equally $1$, $W_{src,dst}=A_{src,dst}=1$. 
In other words, neighbor aggregation weight of a typical GCN is determined solely by the edge degree of source and destination nodes, $-\frac{1}{\sqrt{\mathcal{N}_{src}}\sqrt{\mathcal{N}_{dst}}}$.
LightGCN and NGCF follow such simple neighbor aggregation scheme.
However, if the weight matrix $W$ is other than a simple adjacency matrix, deriving normalized neighbor aggregation weights is computationally expensive because it is not simply decided by the edge degree of source and target nodes. 
In this regard, GNN methods such as GAT or GraphSage applies neighbor aggregation weight in terms of each target node under inductive manner\,(i.e., neighbor aggregation weights sum to $1$ for each node).

\subsection{Plans}
We have two ways to derive neighbor aggregation weight for LightGCN.
\begin{itemize}
    \item Transductive: derive $L^{sym}_{src, dst}$ in Eq.\eqref{eq:Laplacian_normalization}.
    \item Inductive manner: normalize weight matrix $W$ for each target node.
\end{itemize}

